Comprehensive Benchmarking of Binary Neural Networks on NVM Crossbar Architectures

Non-volatile memory (NVM) crossbars have been identified as a promising technology, for accelerating important machine learning operations, with matrix-vector multiplication being a key example. Binary neural networks (BNNs) are especially well-suited for use with NVM crossbars due to their use of a low-bitwidth representation for both activations and weights. However, the aggressive quantization of BNNs can result in suboptimal accuracy, and the analog effects of NVM crossbars can further degrade the accuracy during inference. This paper presents a comprehensive study that benchmarks BNNs trained and validated on ImageNet and deployed on NeuroSim, a simulator for NVM-crossbar-based PIM architecture. Our study analyzes the impact of various parameters, such as input precision and ADC resolution, on both the accuracy of the inference and the hardware performance metrics. We have found that an ADC resolution of 8-bit with an input precision of 4-bit achieves near-optimal accuracy compared to the original BNNs. In addition, we have identified bottleneck components in the PIM architecture that affect area, latency, and energy consumption, and we demonstrate the impact that different BNN layers have on hardware performance.

==> Assets/hw/area/alexnet.tex <==
\begin{tabular}{p{30pt}p{40pt}p{60pt}p{60pt}p{70pt}p{80pt}p{70pt}}
    \hline
        \textbf{ADCprec} & \textbf{ChipArea ($um^2$)} & \textbf{Chip total CIM array ($um^2$)} & \textbf{Total IC Area on chip ($um^2$)} & \textbf{Total ADC (or S/As and precharger for SRAM) Area on chip ($um^2$)} & \textbf{Total Accumulation Circuits (subarray level: adders, shiftAdds; PE/Tile/Global level: accumulation units) on chip ($um^2$)} & \textbf{Other Peripheries (e.g. decoders, mux, switchmatrix, buffers, pooling and activation units) ($um^2$)} \\ \hline
        \textbf{3} & 5.59671E+07 & 4.32399E+06 & 2.53745E+06 & 7.40461E+06 & 1.04988E+06 & 4.06511E+07 \\ 
        \textbf{4} & 6.49219E+07 & 4.32399E+06 & 2.73786E+06 & 1.5867E+07 & 1.21068E+06 & 4.07824E+07 \\ 
        \textbf{5} & 8.26233E+07 & 4.32399E+06 & 3.09679E+06 & 3.27918E+07 & 1.37148E+06 & 4.10392E+07 \\ 
        \textbf{6} & 1.30041E+08 & 4.32399E+06 & 3.90095E+06 & 7.85595E+07 & 1.53228E+06 & 4.17242E+07 \\ 
        \textbf{7} & 2.36966E+08 & 4.32399E+06 & 5.28693E+06 & 1.82391E+08 & 1.69308E+06 & 4.3271E+07 \\ 
        \textbf{8} & 5.73526E+08 & 4.32399E+06 & 8.25709E+06 & 5.10937E+08 & 1.85388E+06 & 4.81535E+07 \\ \hline
    \end{tabular}

==> Assets/hw/area/densenet.tex <==
\begin{tabular}{p{30pt}p{40pt}p{60pt}p{60pt}p{70pt}p{80pt}p{70pt}}
    \hline
        \textbf{ADCprec} & \textbf{ChipArea ($um^2$)} & \textbf{Chip total CIM array ($um^2$)} & \textbf{Total IC Area on chip ($um^2$)} & \textbf{Total ADC (or S/As and precharger for SRAM) Area on chip ($um^2$)} & \textbf{Total Accumulation Circuits (subarray level: adders, shiftAdds; PE/Tile/Global level: accumulation units) on chip ($um^2$)} & \textbf{Other Peripheries (e.g. decoders, mux, switchmatrix, buffers, pooling and activation units) ($um^2$)} \\ \hline
        \textbf{3} & 6.27318E+07 & 4.53715E+06 & 2.66254E+06 & 7.76963E+06 & 1.07889E+06 & 4.66836E+07 \\ 
        \textbf{4} & 7.21264E+07 & 4.53715E+06 & 2.87282E+06 & 1.66492E+07 & 1.24587E+06 & 4.68213E+07 \\ 
        \textbf{5} & 9.06987E+07 & 4.53715E+06 & 3.24945E+06 & 3.44083E+07 & 1.41286E+06 & 4.70908E+07 \\ 
        \textbf{6} & 1.40452E+08 & 4.53715E+06 & 4.09325E+06 & 8.24322E+07 & 1.57985E+06 & 4.78096E+07 \\ 
        \textbf{7} & 2.52647E+08 & 4.53715E+06 & 5.54756E+06 & 1.91382E+08 & 1.74683E+06 & 4.94327E+07 \\ 
        \textbf{8} & 6.05795E+08 & 4.53715E+06 & 8.66413E+06 & 5.36124E+08 & 1.91382E+06 & 5.45559E+07 \\ \hline
    \end{tabular}

==> Assets/hw/area/resnet.tex <==
\begin{tabular}{p{30pt}p{40pt}p{60pt}p{60pt}p{70pt}p{80pt}p{70pt}}
    \hline
        \textbf{ADCprec} & \textbf{ChipArea ($um^2$)} & \textbf{Chip total CIM array ($um^2$)} & \textbf{Total IC Area on chip ($um^2$)} & \textbf{Total ADC (or S/As and precharger for SRAM) Area on chip ($um^2$)} & \textbf{Total Accumulation Circuits (subarray level: adders, shiftAdds; PE/Tile/Global level: accumulation units) on chip ($um^2$)} & \textbf{Other Peripheries (e.g. decoders, mux, switchmatrix, buffers, pooling and activation units) ($um^2$)} \\ \hline
        \textbf{3} & 3.27289E+07 & 2.3447E+06 & 2.52017E+06 & 4.01518E+06 & 5.66319E+05 & 2.32826E+07 \\ 
        \textbf{4} & 3.76747E+07 & 2.3447E+06 & 2.71912E+06 & 8.60395E+06 & 6.53215E+05 & 2.33537E+07 \\ 
        \textbf{5} & 4.74348E+07 & 2.3447E+06 & 3.07544E+06 & 1.77815E+07 & 7.40112E+05 & 2.3493E+07 \\ 
        \textbf{6} & 7.3509E+07 & 2.3447E+06 & 3.87371E+06 & 4.25992E+07 & 8.27009E+05 & 2.38644E+07 \\ 
        \textbf{7} & 1.32114E+08 & 2.3447E+06 & 5.2496E+06 & 9.89022E+07 & 9.13905E+05 & 2.47032E+07 \\ 
        \textbf{8} & 3.15952E+08 & 2.3447E+06 & 8.19816E+06 & 2.77057E+08 & 1.0008E+06 & 2.73508E+07 \\ \hline
    \end{tabular}

==> Assets/hw/densenet.tex <==
\begin{tabular}{ccccccc}
    \hline
        \textbf{ADCprec} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} \\ \hline
        ChipArea (um\^2) & 62731800 & 72126400 & 90698700 & 140452000 & 252647000 & 605795000 \\ 
        Chip total CIM array (um\^2) & 4537150 & 4537150 & 4537150 & 4537150 & 4537150 & 4537150 \\ 
        Total IC Area on chip (um\^2) & 2662540 & 2872820 & 3249450 & 4093250 & 5547560 & 8664130 \\ 
        Total ADC (or S/As and precharger for SRAM) Area on chip (um\^2) & 7769630 & 16649200 & 34408300 & 82432200 & 191382000 & 536124000 \\ 
        Total Accumulation Circuits (subarray level: adders, shiftAdds; PE/Tile/Global level: accumulation units) on chip (um\^2) & 1078890 & 1245870 & 1412860 & 1579850 & 1746830 & 1913820 \\ 
        Other Peripheries (e.g. decoders, mux, switchmatrix, buffers, pooling and activation units) (um\^2) & 46683600 & 46821300 & 47090800 & 47809600 & 49432700 & 54555900 \\ 
        Chip clock period (ns) & 1.96031 & 1.99672 & 2.06768 & 2.20826 & 2.48858 & 3.04875 \\ 
        Chip pipeline-system-clock-cycle (per image) (ns) & 2112010 & 2148370 & 2231700 & 2393210 & 2717680 & 3559270 \\ 
        Chip pipeline-system readDynamicEnergy (per image) (pJ) & 107227000 & 114147000 & 126293000 & 152828000 & 201221000 & 312226000 \\ 
        Chip pipeline-system leakage Energy (per image) (pJ) & 929519 & 1071510 & 1353770 & 1949650 & 3352130 & 7401220 \\ 
        Chip pipeline-system leakage Power (uW) & 539.728 & 611.657 & 746.214 & 1011.91 & 1551.63 & 2662.93 \\ 
        Chip pipeline-system buffer readLatency (per image) (ns) & 1951910 & 1967510 & 2020300 & 2142680 & 2400610 & 2926400 \\ 
        Chip pipeline-system buffer readDynamicEnergy (per image) (pJ) & 2201970 & 2315640 & 2429300 & 2543100 & 2656930 & 2770910 \\ 
        Chip pipeline-system ic readLatency (per image) (ns) & 271983 & 278490 & 321044 & 444284 & 652458 & 1235660 \\ 
        Chip pipeline-system ic readDynamicEnergy (per image) (pJ) & 65284800 & 70967300 & 81106500 & 104098000 & 145869000 & 244089000 \\ 
        ADC (or S/As and precharger for SRAM) readLatency (ns) & 5716.25 & 5822.43 & 6029.35 & 6439.28 & 7256.69 & 8890.15 \\ 
        Accumulation Circuits (subarray level: adders, shiftAdds; PE/Tile/Global level: accumulation units) readLatency (ns) & 68595 & 72780.4 & 78381.6 & 83710.6 & 94337 & 115572 \\ 
        Other Peripheries (e.g. decoders, mux, switchmatrix, buffers, IC, pooling and activation units) readLatency (ns) & 2014380 & 2109820 & 2179490 & 2337450 & 2654850 & 3482290 \\ 
        ADC (or S/As and precharger for SRAM) readDynamicEnergy (pJ) & 32024400 & 32799900 & 34343300 & 37424300 & 43583600 & 55906100 \\ 
        Accumulation Circuits (subarray level: adders, shiftAdds; PE/Tile/Global level: accumulation units) readDynamicEnergy (pJ) & 2332220 & 2681160 & 3030110 & 3379050 & 3728000 & 4076940 \\ 
        Other Peripheries (e.g. decoders, mux, switchmatrix, buffers, IC, pooling and activation units) readDynamicEnergy (pJ) & 72870100 & 78666400 & 88919200 & 112025000 & 153910000 & 252243000 \\ 
        Energy Efficiency TOPS/W & 62.81 & 58.9599 & 53.2196 & 43.8906 & 33.2071 & 21.2538 \\ 
        Throughput TOPS & 3.92414 & 3.85772 & 3.71368 & 3.46305 & 3.04959 & 2.32852 \\ 
        Throughput FPS & 473.483 & 465.469 & 448.089 & 417.849 & 367.961 & 280.957 \\ 
        Compute efficiency TOPS/mm\^2 & 0.0625542 & 0.0534856 & 0.0409453 & 0.0246565 & 0.0120706 & 0.00384374 \\ \hline
    \end{tabular}

==> Assets/hw/efficiency/alexnet.tex <==
\renewcommand\arraystretch{1.5}
\begin{tabular}{ccccc} %p{30pt}p{60pt}p{60pt}p{60pt}p{60pt}
    \hline
        \textbf{ADCprec} & \textbf{Energy Efficiency (TOPS/W)} & \textbf{Throughput (TOPS)} & \textbf{Throughput (FPS)} & \textbf{Compute efficiency (TOPS/$mm^2$)} \\ \hline
        \textbf{3} & 7.99877E+01 & 4.24415E-01 & 1.09713E+02 & 7.5833E-03 \\ 
        \textbf{4} & 7.42018E+01 & 4.17172E-01 & 1.07841E+02 & 6.42576E-03 \\ 
        \textbf{5} & 6.56408E+01 & 4.00355E-01 & 1.03494E+02 & 4.84555E-03 \\ 
        \textbf{6} & 5.22637E+01 & 3.67941E-01 & 9.51146E+01 & 2.82943E-03 \\ 
        \textbf{7} & 3.73681E+01 & 3.20041E-01 & 8.27321E+01 & 1.35058E-03 \\ 
        \textbf{8} & 2.18237E+01 & 2.37037E-01 & 6.12752E+01 & 4.13298E-04 \\ \hline
    \end{tabular}

==> Assets/hw/efficiency/densenet.tex <==
\renewcommand\arraystretch{1.5}
\begin{tabular}{ccccc} %p{30pt}p{60pt}p{60pt}p{60pt}p{60pt}
    \hline
        \textbf{ADCprec} & \textbf{Energy Efficiency (TOPS/W)} & \textbf{Throughput (TOPS)} & \textbf{Throughput (FPS)} & \textbf{Compute efficiency (TOPS/$mm^2$)} \\ \hline
        \textbf{3} & 6.281E+01 & 3.92414E+00 & 4.73483E+02 & 6.25542E-02 \\ 
        \textbf{4} & 5.89599E+01 & 3.85772E+00 & 4.65469E+02 & 5.34856E-02 \\ 
        \textbf{5} & 5.32196E+01 & 3.71368E+00 & 4.48089E+02 & 4.09453E-02 \\ 
        \textbf{6} & 4.38906E+01 & 3.46305E+00 & 4.17849E+02 & 2.46565E-02 \\ 
        \textbf{7} & 3.32071E+01 & 3.04959E+00 & 3.67961E+02 & 1.20706E-02 \\ 
        \textbf{8} & 2.12538E+01 & 2.32852E+00 & 2.80957E+02 & 3.84374E-03 \\ \hline
    \end{tabular}

==> Assets/hw/efficiency/resnet.tex <==
\renewcommand\arraystretch{1.5}
\begin{tabular}{ccccc} %p{30pt}p{60pt}p{60pt}p{60pt}p{60pt}
    \hline
        \textbf{ADCprec} & \textbf{Energy Efficiency (TOPS/W)} & \textbf{Throughput (TOPS)} & \textbf{Throughput (FPS)} & \textbf{Compute efficiency (TOPS/$mm^2$)} \\ \hline
        \textbf{3} & 1.37366E+02 & 2.72123E+00 & 4.95463E+02 & 8.31443E-02 \\ 
        \textbf{4} & 1.28202E+02 & 2.67534E+00 & 4.87108E+02 & 7.10114E-02 \\ 
        \textbf{5} & 1.14779E+02 & 2.57529E+00 & 4.68893E+02 & 5.42913E-02 \\ 
        \textbf{6} & 9.33413E+01 & 2.40165E+00 & 4.37278E+02 & 3.26716E-02 \\ 
        \textbf{7} & 6.89562E+01 & 2.11489E+00 & 3.85065E+02 & 1.60081E-02 \\ 
        \textbf{8} & 4.23204E+01 & 1.61102E+00 & 2.93324E+02 & 5.09893E-03 \\ \hline
    \end{tabular}

==> Assets/hw/latency/alexnet.tex <==
\begin{tabular}{p{30pt}p{50pt}p{50pt}p{60pt}p{60pt}p{60pt}p{70pt}p{70pt}}
    \hline
        \textbf{ADCprec} & \textbf{Chip clock period (ns)} & \textbf{Chip pipeline-system-clock-cycle (per image) (ns)} & \textbf{Chip pipeline-system buffer readLatency (per image) (ns)} & \textbf{Chip pipeline-system ic readLatency (per image) (ns)} & \textbf{ADC (or S/As and precharger for SRAM) readLatency (ns)} & \textbf{Accumulation Circuits (subarray level: adders, shiftAdds; PE/Tile/Global level: accumulation units) readLatency (ns)} & \textbf{Other Peripheries (e.g. decoders, mux, switchmatrix, buffers, IC, pooling and activation units) readLatency (ns)} \\ \hline
        \textbf{3} & 1.96031E+00 & 9.11467E+06 & 8.05026E+06 & 8.73567E+05 & 1.12218E+04 & 1.34661E+05 & 8.96879E+06 \\ 
        \textbf{4} & 1.99672E+00 & 9.27291E+06 & 8.12015E+06 & 9.12654E+05 & 1.14302E+04 & 1.82884E+05 & 9.0786E+06 \\ 
        \textbf{5} & 2.06768E+00 & 9.66243E+06 & 8.3427E+06 & 1.02374E+06 & 1.18364E+04 & 2.36729E+05 & 9.41386E+06 \\ 
        \textbf{6} & 2.20826E+00 & 1.05136E+07 & 8.85219E+06 & 1.29477E+06 & 1.26412E+04 & 3.03388E+05 & 1.01976E+07 \\ 
        \textbf{7} & 2.48858E+00 & 1.20872E+07 & 9.92169E+06 & 1.7523E+06 & 1.42459E+04 & 3.41901E+05 & 1.17311E+07 \\ 
        \textbf{8} & 3.04875E+00 & 1.63198E+07 & 1.20988E+07 & 3.71477E+06 & 1.74526E+04 & 4.18862E+05 & 1.58835E+07 \\ \hline
    \end{tabular}

==> Assets/hw/latency/densenet.tex <==
\begin{tabular}{p{30pt}p{50pt}p{50pt}p{60pt}p{60pt}p{60pt}p{70pt}p{70pt}}
    \hline
        \textbf{ADCprec} & \textbf{Chip clock period (ns)} & \textbf{Chip pipeline-system-clock-cycle (per image) (ns)} & \textbf{Chip pipeline-system buffer readLatency (per image) (ns)} & \textbf{Chip pipeline-system ic readLatency (per image) (ns)} & \textbf{ADC (or S/As and precharger for SRAM) readLatency (ns)} & \textbf{Accumulation Circuits (subarray level: adders, shiftAdds; PE/Tile/Global level: accumulation units) readLatency (ns)} & \textbf{Other Peripheries (e.g. decoders, mux, switchmatrix, buffers, IC, pooling and activation units) readLatency (ns)} \\ \hline
        \textbf{3} & 1.96031E+00 & 2.11201E+06 & 1.95191E+06 & 2.71983E+05 & 5.71625E+03 & 6.8595E+04 & 2.01438E+06 \\ 
        \textbf{4} & 1.99672E+00 & 2.14837E+06 & 1.96751E+06 & 2.7849E+05 & 5.82243E+03 & 7.27804E+04 & 2.10982E+06 \\ 
        \textbf{5} & 2.06768E+00 & 2.2317E+06 & 2.0203E+06 & 3.21044E+05 & 6.02935E+03 & 7.83816E+04 & 2.17949E+06 \\ 
        \textbf{6} & 2.20826E+00 & 2.39321E+06 & 2.14268E+06 & 4.44284E+05 & 6.43928E+03 & 8.37106E+04 & 2.33745E+06 \\ 
        \textbf{7} & 2.48858E+00 & 2.71768E+06 & 2.40061E+06 & 6.52458E+05 & 7.25669E+03 & 9.4337E+04 & 2.65485E+06 \\ 
        \textbf{8} & 3.04875E+00 & 3.55927E+06 & 2.9264E+06 & 1.23566E+06 & 8.89015E+03 & 1.15572E+05 & 3.48229E+06 \\ \hline
    \end{tabular}

==> Assets/hw/latency/resnet.tex <==
\begin{tabular}{p{30pt}p{50pt}p{50pt}p{60pt}p{60pt}p{60pt}p{70pt}p{70pt}}
    \hline
        \textbf{ADCprec} & \textbf{Chip clock period (ns)} & \textbf{Chip pipeline-system-clock-cycle (per image) (ns)} & \textbf{Chip pipeline-system buffer readLatency (per image) (ns)} & \textbf{Chip pipeline-system ic readLatency (per image) (ns)} & \textbf{ADC (or S/As and precharger for SRAM) readLatency (ns)} & \textbf{Accumulation Circuits (subarray level: adders, shiftAdds; PE/Tile/Global level: accumulation units) readLatency (ns)} & \textbf{Other Peripheries (e.g. decoders, mux, switchmatrix, buffers, IC, pooling and activation units) readLatency (ns)} \\ \hline
        \textbf{3} & 1.96031E+00 & 2.01831E+06 & 1.85961E+06 & 1.20835E+05 & 5.71625E+03 & 6.00207E+04 & 1.99211E+06 \\ 
        \textbf{4} & 1.99672E+00 & 2.05293E+06 & 1.87349E+06 & 1.2901E+05 & 5.82243E+03 & 6.11356E+04 & 2.01438E+06 \\ 
        \textbf{5} & 2.06768E+00 & 2.13268E+06 & 1.92294E+06 & 1.45232E+05 & 6.02935E+03 & 6.63229E+04 & 2.08048E+06 \\ 
        \textbf{6} & 2.20826E+00 & 2.28688E+06 & 2.03871E+06 & 1.79274E+05 & 6.43928E+03 & 7.0832E+04 & 2.23112E+06 \\ 
        \textbf{7} & 2.48858E+00 & 2.59696E+06 & 2.28344E+06 & 2.35882E+05 & 7.25669E+03 & 7.98236E+04 & 2.53413E+06 \\ 
        \textbf{8} & 3.04875E+00 & 3.4092E+06 & 2.78285E+06 & 5.31239E+05 & 8.89015E+03 & 9.77917E+04 & 3.33223E+06 \\ \hline
    \end{tabular}

==> Assets/hw/power/alexnet.tex <==
\begin{tabular}{p{30pt}p{50pt}p{50pt}p{60pt}p{60pt}p{60pt}p{70pt}p{70pt}p{70pt}}
    \hline
        \textbf{ADCprec} & \textbf{Chip pipeline-system readDynamicEnergy (per image) (pJ)} & \textbf{Chip pipeline-system leakage Energy (per image) (pJ)} & \textbf{Chip pipeline-system leakage Power (uW)} & \textbf{Chip pipeline-system buffer readDynamicEnergy (per image) (pJ)} & \textbf{Chip pipeline-system ic readDynamicEnergy (per image) (pJ)} & \textbf{ADC (or S/As and precharger for SRAM) readDynamicEnergy (pJ)} & \textbf{Accumulation Circuits (subarray level: adders, shiftAdds; PE/Tile/Global level: accumulation units) readDynamicEnergy (pJ)} & \textbf{Other Peripheries (e.g. decoders, mux, switchmatrix, buffers, IC, pooling and activation units) readDynamicEnergy (pJ)} \\ \hline
        \textbf{3} & 3.48921E+07 & 4.74922E+06 & 5.54641E+02 & 8.56618E+05 & 2.36371E+07 & 9.17445E+06 & 4.01664E+05 & 2.5316E+07 \\ 
        \textbf{4} & 3.7249E+07 & 5.48334E+06 & 6.29465E+02 & 9.04675E+05 & 2.57391E+07 & 9.34475E+06 & 4.38153E+05 & 2.74661E+07 \\ 
        \textbf{5} & 4.13709E+07 & 6.93481E+06 & 7.63976E+02 & 9.52543E+05 & 2.94692E+07 & 9.65198E+06 & 4.74641E+05 & 3.12442E+07 \\ 
        \textbf{6} & 5.05601E+07 & 1.01095E+07 & 1.02346E+03 & 1.00047E+06 & 3.7896E+07 & 1.03301E+07 & 5.11129E+05 & 3.97189E+07 \\ 
        \textbf{7} & 6.73163E+07 & 1.75375E+07 & 1.54411E+03 & 1.04882E+06 & 5.32089E+07 & 1.16885E+07 & 5.47617E+05 & 5.50801E+07 \\ 
        \textbf{8} & 1.05269E+08 & 4.00235E+07 & 2.60947E+03 & 1.09684E+06 & 8.92288E+07 & 1.35353E+07 & 5.84105E+05 & 9.11499E+07 \\ \hline
    \end{tabular}

==> Assets/hw/power/densenet.tex <==
\begin{tabular}{p{30pt}p{50pt}p{50pt}p{60pt}p{60pt}p{60pt}p{70pt}p{70pt}p{70pt}}
    \hline
        \textbf{ADCprec} & \textbf{Chip pipeline-system readDynamicEnergy (per image) (pJ)} & \textbf{Chip pipeline-system leakage Energy (per image) (pJ)} & \textbf{Chip pipeline-system leakage Power (uW)} & \textbf{Chip pipeline-system buffer readDynamicEnergy (per image) (pJ)} & \textbf{Chip pipeline-system ic readDynamicEnergy (per image) (pJ)} & \textbf{ADC (or S/As and precharger for SRAM) readDynamicEnergy (pJ)} & \textbf{Accumulation Circuits (subarray level: adders, shiftAdds; PE/Tile/Global level: accumulation units) readDynamicEnergy (pJ)} & \textbf{Other Peripheries (e.g. decoders, mux, switchmatrix, buffers, IC, pooling and activation units) readDynamicEnergy (pJ)} \\ \hline
        \textbf{3} & 1.07227E+08 & 9.29519E+05 & 5.39728E+02 & 2.20197E+06 & 6.52848E+07 & 3.20244E+07 & 2.33222E+06 & 7.28701E+07 \\ 
        \textbf{4} & 1.14147E+08 & 1.07151E+06 & 6.11657E+02 & 2.31564E+06 & 7.09673E+07 & 3.27999E+07 & 2.68116E+06 & 7.86664E+07 \\ 
        \textbf{5} & 1.26293E+08 & 1.35377E+06 & 7.46214E+02 & 2.4293E+06 & 8.11065E+07 & 3.43433E+07 & 3.03011E+06 & 8.89192E+07 \\ 
        \textbf{6} & 1.52828E+08 & 1.94965E+06 & 1.01191E+03 & 2.5431E+06 & 1.04098E+08 & 3.74243E+07 & 3.37905E+06 & 1.12025E+08 \\ 
        \textbf{7} & 2.01221E+08 & 3.35213E+06 & 1.55163E+03 & 2.65693E+06 & 1.45869E+08 & 4.35836E+07 & 3.728E+06 & 1.5391E+08 \\ 
        \textbf{8} & 3.12226E+08 & 7.40122E+06 & 2.66293E+03 & 2.77091E+06 & 2.44089E+08 & 5.59061E+07 & 4.07694E+06 & 2.52243E+08 \\ \hline
    \end{tabular}

==> Assets/hw/power/resnet.tex <==
\begin{tabular}{p{30pt}p{50pt}p{50pt}p{60pt}p{60pt}p{60pt}p{70pt}p{70pt}p{70pt}}
    \hline
        \textbf{ADCprec} & \textbf{Chip pipeline-system readDynamicEnergy (per image) (pJ)} & \textbf{Chip pipeline-system leakage Energy (per image) (pJ)} & \textbf{Chip pipeline-system leakage Power (uW)} & \textbf{Chip pipeline-system buffer readDynamicEnergy (per image) (pJ)} & \textbf{Chip pipeline-system ic readDynamicEnergy (per image) (pJ)} & \textbf{ADC (or S/As and precharger for SRAM) readDynamicEnergy (pJ)} & \textbf{Accumulation Circuits (subarray level: adders, shiftAdds; PE/Tile/Global level: accumulation units) readDynamicEnergy (pJ)} & \textbf{Other Peripheries (e.g. decoders, mux, switchmatrix, buffers, IC, pooling and activation units) readDynamicEnergy (pJ)} \\ \hline
        \textbf{3} & 3.22658E+07 & 5.07125E+05 & 2.93543E+02 & 8.28566E+05 & 1.83887E+07 & 1.09578E+07 & 5.33442E+05 & 2.07746E+07 \\ 
        \textbf{4} & 3.453E+07 & 5.85325E+05 & 3.32984E+02 & 8.91473E+05 & 2.01852E+07 & 1.12858E+07 & 6.10198E+05 & 2.26341E+07 \\ 
        \textbf{5} & 3.84833E+07 & 7.38685E+05 & 4.04791E+02 & 9.54403E+05 & 2.33677E+07 & 1.19171E+07 & 6.86955E+05 & 2.58792E+07 \\ 
        \textbf{6} & 4.71674E+07 & 1.06288E+06 & 5.44366E+02 & 1.01737E+06 & 3.06151E+07 & 1.32138E+07 & 7.63711E+05 & 3.31899E+07 \\ 
        \textbf{7} & 6.34608E+07 & 1.82517E+06 & 8.25554E+02 & 1.0804E+06 & 4.4205E+07 & 1.57774E+07 & 8.40467E+05 & 4.68429E+07 \\ 
        \textbf{8} & 1.02321E+08 & 4.0551E+06 & 1.40212E+03 & 1.14349E+06 & 7.77896E+07 & 2.09134E+07 & 9.17224E+05 & 8.04903E+07 \\ \hline
    \end{tabular}

==> Assets/test/test_table.tex <==
\renewcommand\arraystretch{1.05}
\begin{tabular}{c|cccccc}
    \toprule
    \multirow{2}{4em}{\centering \textbf{Input Precision}} &\multicolumn{6}{c}{\textbf{ADC Resolution}} \\
    ~ & {3} & {4} & {5}& {6}& {7} & {8}  \\ 
    \midrule
    {1} & 0.17 & 1.43 & 3.64 & 6.07 & 7.67 & 7.55 \\ 
    {2} & 0.17 & 3.03 & 9.27 & 22.58 & 29.97 & 30.71 \\ 
    {3} & 0.21 & 4.35 & 13.81 & 29.30 & 34.84 & 35.60 \\ 
    {4} & 0.16 & 4.95 & 15.51 & 30.76 & 35.57 & 35.76 \\ 
    {5} & 0.15 & 5.18 & 15.96 & 31.06 & 35.52 & 36.11 \\ 
    {6} & 0.18 & 5.24 & 16.00 & 30.99 & 35.54 & 35.84 \\ 
    {7} & 0.29 & 5.31 & 16.18 & 31.28 & 35.43 & 35.90 \\ 
    {8} & 0.31 & 5.31 & 16.31 & 31.22 & 35.56 & 35.90 \\
    \bottomrule
\end{tabular}
